Optical Networks and Interconnects

The rapid evolution of communication technologies such as 5G and beyond, rely on optical networks to support the challenging and ambitious requirements that include both capacity and reliability. This chapter begins by giving an overview of the evolution of optical access networks, focusing on Passive Optical Networks (PONs). The development of the different PON standards and requirements aiming at longer reach, higher client count and delivered bandwidth are presented. PON virtualization is also introduced as the flexibility enabler. Triggered by the increase of bandwidth supported by access and aggregation network segments, core networks have also evolved, as presented in the second part of the chapter. Scaling the physical infrastructure requires high investment and hence, operators are considering alternatives to optimize the use of the existing capacity. This chapter introduces different planning problems such as Routing and Spectrum Assignment problems, placement problems for regenerators and wavelength converters, and how to offer resilience to different failures. An overview of control and management is also provided. Moreover, motivated by the increasing importance of data storage and data processing, this chapter also addresses different aspects of optical data center interconnects. Data centers have become critical infrastructure to operate any service. They are also forced to take advantage of optical technology in order to keep up with the growing capacity demand and power consumption. This chapter gives an overview of different optical data center network architectures as well as some expected directions to improve the resource utilization and increase the network capacity.

==> Handbook chapter/reference_CM.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% reference.tex %%%%%%%%%%%%%%%%%%%%%
% sample references
% 
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\begin{thebibliography}{99.}
\bibitem{FTTH_77} Kawahata M. (1977) Hi-OVIS (Higashi Ikoma optical visual information System) development project. in Proc. Integ. Optics and Optical Commun. (IOOC.77), 1977, pp. 467-471.
\bibitem{UDWDM} Li J. et al. (2018) Real-time bidirectional coherent ultra-dense TWDM-PON for 1000 ONUs. Opt. Express 26, 22976-22984 
\bibitem{Hill_90} Hill A. M. et al. (1990) 39.5 million-way WDM broadcast network employing two stages of erbium-doped fibre amplifiers. Electronics Letters 26: 1882-1884.
\bibitem{LR-PON} Ruffini M. et al. (2017) Access and metro network convergence for flexible end to end network design.  IEEE/OSA Journal of Communications and Networking, Vol. 9, No. 6, June 2017.
\bibitem{Flat-core} Raack C. et al. (2016) Hierarchical Versus Flat Optical Metro/Core Networks: A Systematic Cost and Migration Study. IEEE Optical Networks Design and Modeling (ONDM), May 2016.
\bibitem{Prot1} Ruffini M. et al. (2010) Protection Strategies for Long-Reach PON. ECOC 2010.
\bibitem{Prot2} McGettrick S. et al. (2016) Experimental End-to-End Demonstration of Shared N:M Dual Homed Protection in SDN-controlled Long Reach PON and Pan-European Core. IEEE/OSA Journal of Lightwave technology, vol. 34, No. 18, September 2016.
\bibitem{LRPON-SOA} Talli G. et al. (2017) SDN Enabled Dynamically Reconfigurable High Capacity Optical Access Architecture for Converged Services.IEEE/OSA Journal of Lightwave technology, Vol. 35, No.3, March 2017.
\bibitem{LRPON-demo} Talli G. et al. (2016) Demonstration of SDN Enabled Dynamically Reconfigurable High Capacity Optical Access for Converged Services. Proc. of Optical Fibre Communications conference (OFC), March 2016, post-deadline paper.
\bibitem{NGMN} NGMN Alliance white paper (2018) NGMN Overview on 5G RAN Functional Decomposition. Available at \url{https://www.ngmn.org/wp-content/uploads/Publications/2018/180226_NGMN_RANFSX_D1_V20_Final.pdf}
\bibitem{PON_backhaul} Alvarez P. et al. (2014) Backhaul Mobile Systems with GPON using Group Assured Bandwidth. IEEE European Conference on Network and Optical Communications (NOC), 2014
\bibitem{ORAN-latency} Umesh A. et al. (2019) Overview of O-RAN fronthaul specification. NTT DOCOMO Tech. J. Vol 21, No 1, 2019. Available at \url{https://www.nttdocomo.co.jp/english/binary/pdf/corporate/technology/rd/technical_journal/bn/vol21_1/vol21_1_007en.pdf}
\bibitem{NTT-OFC-2014}Tashiro T. et al. (2014) A novel DBA scheme for TDM-PON based mobile fronthaul. OFC 2014, paper Tu3F.3
\bibitem{CTI} O-RAN Fronthaul Cooperative Transport Interface Transport Control Plane Specification 1.0 - April 2020 (O-RAN.WG4.CTI-TCP.0-v01.00)
\bibitem{Intra-ONU1} Ranaweera C. et al. (2012) Next generation optical-wireless converged network architectures. IEEE Network 26, 22?-27.
\bibitem{Intra-ONU2} Li J. and Chen J. (2017) Passive optical network based mobile backhaul enabling ultra-low latency for communications among base stations. IEEE/OSA Journal of Optical Communications and Networking 9, 855-863
\bibitem{MESH-PON} Das S. and Ruffini M. (2020) PON Virtualisation with EAST-WEST Communications for Low-Latency Converged Multi-Access Edge Computing (MEC). OFC 2020.
\bibitem{MESH-experiment} Das S. et al. (2020) Virtualised EAST-WEST PON Architecture Supporting Low-Latency communication for Mobile Functional-Split Based on Multi-Access Edge Computing. OSA Journal of Optical Communications and Networking, No 10, Vol 12, October 2020.
\bibitem{Cloud-access} Ruffini M. and Slyne F. (2019) Moving the Network to the Cloud: the Cloud Central Office Revolution and its Implications for the Optical Layer. IEEE/OSA Journal of Lightwave Technology, Vol. 37, No 7, April 2019.
\bibitem{CORD} Peterson L. et al. (2016) Central office re-architected as a data center.  IEEE Communications Magazine, vol. 54, no. 10, pp. 96-101, 2016.
\bibitem{DT-SEBA} https://techblog.comsoc.org/2021/01/28/deutsche-telekom-access-4-0-in-production-leveraging-onf-voltha-and-seba-open-source-software/
\bibitem{FASA} Asaka K. et al. (2018) Flexible access system architecture (FASA). OFC 2018, paper Tu3L.7.
\bibitem{BBF-402}  Functional model for PON abstraction interface. TR-402 Standard BroadBand Forum (BBF), 2018.
\bibitem{vDBA-concept} Elrasad A. et al. (2017) Virtual Dynamic Bandwidth Allocation Enabling True PON Multi-Tenancy. OFC 2017, paper M3I.3.
\bibitem{vDBA-test} Ruffini M. et al. (2020) The Virtual DBA: Virtualizing Passive Optical Networks to Enable Multi-Service Operation in True Multi-Tenant Environments. OSA Journal of Optical Communications and Networking, No.4, Vol.12, April 2020.
\bibitem{BBF-370} BBF TR-370i2 Fixed Access Network Sharing - Architecture and Nodal Requirements, issue 2. Publication planned in 2020.
\bibitem{OFC-21} Slyne F. et al. (2021) Stateful DBA Hypervisor Supporting SLAs with Low Latency \& High Availability in Shared PON. To appear in OFC, June 2021.
\bibitem{Patri2021} C. Mas-Machuca et al. (2022) Long-term Capacity Planning in Flexible Optical Transport Networks. Optical Fiber Communication Conference (OFC), 2022
\bibitem{Amir2021} A. Varasteh, et al. (2021) Towards Dynamic Network Reconfigurations for Flexible Optical Network Planning. Optical Fiber Communication Conference (OFC), 2021.
\bibitem{EUReport} Annual Incident Reports 2015 (2016) European Union Agency For Network And Information Security
\bibitem{OFReport} Reliability of fiber optical cable systems (2001) ALCOA FUJIKURA LTD.
\bibitem{SNDlib} SNDlib library (2006) \url{http://sndlib.zib.de/}
\bibitem{Li2018} Li J. et al. (2018) Real-time bidirectional coherent ultra-dense TWDM-PON for 1000 ONUs Vol. 26, No. 18 | 3 Sep 2018 | OPTICS EXPRESS 22978 
%\bibitem{Fawaz2010} W. Fawaz and K. Chen Survivability 
\bibitem{Liu2013} Liu M. et al. (2013) Survivable traffic grooming in elastic optical networks - Shared protection Journal of Lightwave Technology 31(6):903-909, 2013
\bibitem{Shen2014} Shen G. et al. (2014) Optimal Design for shared backup path protected elastic optical networks under single-link failure Journal of Optical Communications and Networking 6(7):649, 2014 
\bibitem{Schupke2002} Schupke D. A. (2002), "Fast and efficient WDM network protection using p-cycles," IEEE/LEOS Summer Topics All-Optical Networking, 2002, doi: 10.1109/LEOSST.2002.1027541.
\bibitem{Ji2013} Ji F. et al. (2013) Dynamic p-cycle configuration in spectrum-sliced elastic optical networks IEEE Global Communications Conference (GLOBECOM)
\bibitem{Kilper2004} Kilper D. C. et al. (2004) "Optical performance monitoring," J. Lightwave Technol. 22, 294.
\bibitem{Mrozek2018} Mrozek T. (2018) "Simultaneous Monitoring of Chromatic Dispersion and Optical Signal to Noise Ratio in Optical Network Using Asynchronous Delay Tap Sampling and Convolutional Neural Network (Deep Learning)," 2018 20th International Conference on Transparent Optical Networks (ICTON), 2018, pp. 1-4, doi: 10.1109/ICTON.2018.8473703.
\bibitem{Isabella2021} Dick I. (2021) Machine Learning based Fault Detection Algorithms for Long Haul Elastic Optical Networks TUM Technical Report May 
\bibitem{Faisal2018}Faisal N. K. et al. (2018) Machine Learning-Assisted Optical Performance Monitoring in Fiber-Optic Networks 2018 IEEE Photonics Society Summer Topical Meeting Series
\bibitem{Shahkarami2018} Shahkarami S. et al. (2018) Machine-Learning-Based Soft-Failure Detection and Identification in Optical Networks 2018 Optical Fiber Communications Conference and Exposition (OFC)
\bibitem{Panayiotou2018}Panayiotou T. et al. (2018) "Leveraging statistical machine learning to address failure localization in optical networks," in IEEE/OSA Journal of Optical Communications and Networking, vol. 10, no. 3, pp. 162-173, March 2018, doi: 10.1364/JOCN.10.000162.
\bibitem{Vela2018} Vela A. P. et al. (2018) "Soft Failure Localization in Elastic Optical Networks," 2018 20th International Conference on Transparent Optical Networks (ICTON), 2018, pp. 1-4, doi: 10.1109/ICTON.2018.8473716.
\bibitem{Assis2019} Assis K. D. R.  et al. (2019) SLA formulation for squeezed protection in elastic optical networks considering the modulation format, in IEEE/OSA Journal of Optical Communications and Networking, vol. 11, no. 5, pp. 202-212, May 2019, doi: 10.1364/JOCN.11.000202.
\bibitem{SLA} Akbari-Moghanjoughi A. et al. (2019) Guidelines to SLA modeling and establishment in heterogeneous communications networks, 2019 21st International Conference on Transparent Optical Networks (ICTON), 2019, pp. 1-4, doi: 10.1109/ICTON.2019.8840537.
\bibitem{Liu2015} Liu L. et al. (2015) Dynamic OpenFlow-Based Lightpath Restoration in Elastic Optical Networks on the GENI Testbed, in Journal of Lightwave Technology, vol. 33, no. 8, pp. 1531-1539, 15 April15, 2015, doi: 10.1109/JLT.2014.2388194.
\bibitem{Papanikolaou2017} Papanikolaou P. et al. (2017)Joint multi-layer survivability techniques for IP-over-elastic-optical- networks," in IEEE/OSA Journal of Optical Communications and Networking, vol. 9, no. 1, pp. A85-A98, Jan. 2017, doi: 10.1364/JOCN.9.000A85.
\bibitem{Chiu2011} Chiu A. L. et al. (2011) Integrated Restoration for Next-Generation IP-Over-Optical Networks, in Journal of Lightwave Technology, vol. 29, no. 6, pp. 916-924, March 2011, doi: 10.1109/JLT.2011.2111354.
\bibitem{WC1} Gao S. et al. (2003) An optimization model for placement of wavelength converters to minimize blocking probability in WDM networks, in Journal of Lightwave Technology, vol. 21, no. 3, pp. 684-694, March 2003, doi: 10.1109/JLT.2003.809584.
\bibitem{WC2} Subramaniam S. et al. (1999) On optimal converter placement in wavelength-routed networks, in IEEE/ACM Transactions on Networking, vol. 7, no. 5, pp. 754-766, Oct. 1999, doi: 10.1109/90.803388.
\bibitem{WC3} Tran P. N. and Killat U. (2008) An Exact ILP Formulation for Optimal Wavelength Converter Usage and Placement in WDM Networks, IEEE GLOBECOM 2008 - 2008 IEEE Global Telecommunications Conference, 2008, pp. 1-6, doi: 10.1109/GLOCOM.2008.ECP.530.
\bibitem{WC4} Wang X. et al. (2015) Impact of wavelength and modulation conversion on translucent elastic optical networks using MILP, in IEEE/OSA Journal of Optical Communications and Networking, vol. 7, no. 7, pp. 644-655, July 2015, doi: 10.1364/JOCN.7.000644.
\bibitem{Boscolo2005} Boscolo S. et al. (2005) Performance comparison of 2R and 3R optical regeneration schemes at 40 Gb/s for application to all-optical networks, in Journal of Lightwave Technology, vol. 23, no. 1, pp. 304-309, Jan. 2005, doi: 10.1109/JLT.2004.834986.
\bibitem{Simmons2008} Simmons J.M. (2008) Regeneration. In: Optical Network Design and Planning. Optical Networks. Springer, Boston, MA.
\bibitem{Khomchenko2021} Khomchenko D. et al. (2021) Transmission-aware Bandwidth Variable Transceiver Allocation in DWDM Optical Networks, ONDM 2021
\bibitem{Saquib2022}S. Amjad et al. (2022) Towards Regeneration in Flexible Optical Network Planning. 26th International Conference on Optical Network Design and Modelling (ONDM 2022) 2022, pp. 1-6, doi: 10.23919/ONDM54585.2022.9782815. 
\bibitem{Cavalcante2019} Cavalcante M.A. et al. (2019) An auxiliary-graph-based methodology for regenerator assignment problem optimization in translucent elastic optical networks, Optical Fiber Technology, Volume 53, 2019,ISSN 1068-5200,https://doi.org/10.1016/j.yofte.2019.102008.
\bibitem{deSilva2020}da Silva E. F. et al. (2020) Assessment of novel regenerator assignment strategies in dynamic translucent elastic optical networks, February 2020, Photonic Network Communications 39(9), DOI: 10.1007/s11107-019-00873-9
\bibitem{Casellas2018} Casellas R. et al. (2018) Control, Management, and Orchestration of Optical Networks: Evolution, Trends, and Challenges, J. Lightwave Technol. 36, 1390-1402 (2018) https://www.osapublishing.org/jlt/abstract.cfm?URI=jlt-36-7-1390
\bibitem{Chin2017} Chin H. et al. (2017) Estimating coherent optical transmission system performance over heterogeneous fibre span lengths, 19th International Conference on Transparent Optical Networks (ICTON), 2017, pp. 1-4, doi: 10.1109/ICTON.2017.8025003.
\bibitem{Sai2020} Patri S. K. et al. (2020) HeCSON: Heuristic for Configuration Selection in Optical Network Planning, 2020 Optical Fiber Communications Conference and Exhibition (OFC), 2020, pp. 1-3.
\bibitem{Achim2011} Autenrieth A. et al. (2011) Power consumption analysis of opaque and transparent optical core networks, 13th International Conference on Transparent Optical Networks, 2011, pp. 1-5, doi: 10.1109/ICTON.2011.5971075.
\bibitem{ISO} Information Technology—Open Systems Interconnection—Systems Management Overview, ISO/IEC 10040, 1998
\bibitem{virt} Zhang J. et al. (2020) Optical Network Virtualization. In: Mukherjee B., Tomkos I., Tornatore M., Winzer P., Zhao Y. (eds) Springer Handbook of Optical Networks. Springer Handbooks. Springer, Cham. 
\bibitem{hyp} Papaioannou A. D. et al.(2016) The Benefits of a Disaggregated Data Centre: A Resource Allocation Approach, IEEE Global Communications Conference (GLOBECOM) 2016 
\bibitem{DC1} Roozbeh A. et al. (2018) Software-defined Hardware Infrastructures: A Survey on Enabling Technologies and Open Research Directions, IEEE Communications Surveys \& Tutorials, Vol. 20, Issue 3, pp. 2454-2485, Sept. 2018
\bibitem{DC2} Chen J. et al. (2015) Optical interconnects at the top of the rack for energy-efficient data centers, in IEEE Communications Magazine, vol. 53, Issue 8, pp. 140-148, Aug. 2015, doi: 10.1109/MCOM.2015.7180521.
\bibitem{DC3}Farrington N.  et al. (2010) Helios: A Hybrid Electrical/Optical Switch Architecture for Modular Data Centers,” in Proc. SIGCOMM’10, New Delhi, India
\bibitem{DC4} Chen J. and Wosinska L. (2021) “Photonics in Intra-Datacenter Networks: Architecture and Future Developments,” in Proc. IEEE/OSA the 26th Optoelectronics and Communications Conference, July 2021
\bibitem{DC5} Chen K. et al. (2014) OSA: An optical switching architecture for data center networks with unprecedented flexibility, in IEEE/ACM Transactions on Networking, Vol. 22, Issue 2, pp. 498–511, Apr. 2014
\bibitem{DC6}Yin Y. et al. (2013) LIONS: An AWGR-Based Low-Latency Optical Switch for High-Performance Computing and Data Centers, in IEEE Journal of Selected Topics in Quantum Electronics, Vol. 19, Issue 2, March-April 2013.
\bibitem{DCF} Fiorani M. et al. (2017) Spatial Division Multiplexing for High Capacity Optical Interconnects in Modular Data Centers, IEEE/OSA Journal of Optical Communication and Networking (JOCN), Vol. 9, Issue 2, pp. A143-A153, February 2017
\bibitem{DC8} Fiorani M. et al. (2014) Energy-Efficient Elastic Optical Interconnect Architecture for Data Centers, in IEEE Communications Letters, vol. 18, Issue 9, pp. 1531-1534, Sept. 2014, doi: 10.1109/LCOMM.2014.2339322
\bibitem{DC7} Cheng Y. et al. (2015) Reliable and Cost Efficient Passive Optical Interconnects for Data Centers, in IEEE Communications Letters, vol. 19, Issue 11, pp. 1913-1916, Nov. 2015, doi: 10.1109/LCOMM.2015.2478474.
\bibitem{DC9} Lin R. et al. (2020) Disaggregated Data Centers: Challenges and Trade-offs, in IEEE Communications Magazine, Vol. 58, Issue 2, pp. 20-26, Feb. 2020 
\bibitem{DC10} Zhang L. et al. (2020) Enabling Technologies for Optical Data Center Networks: Spatial Division Multiplexing, (Invited Tutorial), in IEEE/OSA Journal of Lightwave Technology (JLT), Print ISSN: 0733-8724, Online ISSN: 1558-2213, DOI: 10.1109/JLT.2019.2941765, Vol. 38, Issue 1, pp. 18 – 30, Jan.. 2020 
%\bibitem{DC11} K. Chen, A. Singla, A. Singh, K. Ramachandran, L. Xu, Y. Zhang, X. Wen, and Y. Chen, “OSA: An optical switching architecture for data center networks with unprecedented flexibility,” in IEEE/ACM Transactions on Networking, Vol. 22, Issue 2, pp. 498–511, Apr. 2014
%\bibitem{DC12} Y. Yin, R. Proietti, X. Ye, C. J. Nitta, V. Akella, and S. J. B. Yoo, “LIONS: An AWGR-Based Low-Latency Optical Switch for High-Performance Computing and Data Centers,” in IEEE journal of Selected Topics in Quantum Electronics (JSTQE), Vol. 19, Issue 2, March-April 2013.
%\bibitem{DC13}M. Xu, C. Liu, and S. Subramaniam, “PODCA: a passive optical data center network architecture”, in IEEE/OSA Journal of Optical Communications and Networking (JOCN), vol. 10, Issue 4, pp. 409-420, April 2018.


% Book Chapter
%\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York, p 234--295  
%
% Online Document
%\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
%\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
%\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
%\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
%\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%

\end{thebibliography}
